Superradiance-assisted two-color Doppler cooling of molecules

For experiments that require a quantum system to be in the ultra-cold regime, laser cooling is an essential tool. While techniques for laser cooling ions and neutral atoms have been refined and temperatures below the Doppler limit have been achieved, present-day techniques are limited to a small class of molecules. This paper proposes a general cooling scheme for molecules based on vibrational-state transitions. Superradiance is used to speed up the two-photon transition. Simulations of this scheme achieve temperatures comparable to those achieved by existing two-level schemes for neutral atoms and ions.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}

